Fermion Bag Approach for Hamiltonian Lattice Field Theories

Two formidable bottlenecks to the applicability of QMC include: (1) the sign problem and (2) algorithmic update inefficiencies. In this thesis, I overcome both these difficulties for a class of problems by extending the fermion bag approach to the Hamiltonian formalism and demonstrating progress using the example of a specific quantum system known as the $t$-$V$ model, which exhibits a transition from a semimetal to an insulator phase for a single flavor of four-component Dirac fermions. The success of this extension is demonstrated in two ways: first, through solutions to sign problems, and second, through the development of new efficient QMC algorithms. In addressing the first point, I present a solution to the sign problem for the aforementioned $t$-$V$ model, which is then extended to many other Hamiltonian models within a class that involves fermions interacting with quantum spins. Some of these models contain an interesting quantum phase transition between a massless/semimetal phase to a massive/insulator phase in the Gross-Neveu universality class. The second point is addressed through the construction of a Hamiltonian fermion bag algorithm, which is then used to compute critical exponents for the second-order phase transition in the $t$-$V$ model and is described in detail here. The largest lattice sizes of $64^2$ at a comparably low temperature are reachable due to efficiency gains from this Hamiltonian fermion bag algorithm. The two independent critical exponents I find, which completely characterize the phase transition, are $\eta=.51(3)$ and $\nu=.89(1)$. The finite size scaling fit is excellent with a $\chi^2/DOF=.90$, showing strong evidence for a second-order critical phase transition, and hence a non-perturbative QFT can be defined at the critical point.

==> CHANGELOG <==
Version 0.4:
Removed features:
* parts. Does not comply with G-school style
* two-column signature page. Can only have up to six members.
* Duke logo
Bug fixes
* fixed double-spacing in List of Tables.

Version 0.3:
New features:
* "oldstyle" returns to the standard LaTeX report style for headings 
* "nobind" centers the text on the page (and it's now on by default in economy) 
Bug fixes
* Fixed dedication format and placement 
* Fixed small spelling errors in dissertation.tex (oops!)
* Fixed single-spacing in body when there are no frontmatter chapters

Version 0.25:
* Fixed bug in 'economy' option not playing nice with other options
* Tweaked section headers to be slightly smaller
* Make \raggedbottom the default page layout to avoid lots of underful vboxes
* ifpdf.sty no longer required
* Added fix_bookmarks.py hack to work-around missing features in hyperref

Version 0.2:
* Fixed warning during compliation from hyperref
* Automatic entry of PDF metadata from title and author fields.
* Citation hyperlinks working (but no more grouped cite support)
* Improved floatpage formatting.
* Support for longer titles, up to four lines

--------------------------------------------------
Version 0.1:
Released to a select audience.  Essentially functional.


==> clusters.tex <==
\begin{tikzpicture}

\draw[draw = white] (1,7.6)--(6,7.6)
node[pos=.5] {\large \textbf{ Isolated:}};

\draw[draw = white] (1,.9)--(6,.9)
node[pos=0] {1}
node[pos=.2] {2}
node[pos=.4] {3}
node[pos=.6]{4}
node[pos=.8]{5}
node[pos=1.0]{6};

\draw[draw = white] (1,7.1)--(6,7.1)
node[pos=0] {1}
node[pos=.2] {2}
node[pos=.4] {3}
node[pos=.6]{4}
node[pos=.8]{5}
node[pos=1.0]{6};    


\draw[ color=blue] (1,1.5) rectangle (6,6.5);

\draw[pattern=north west lines, pattern color=blue] (2,2.5) rectangle (3,4);
\draw[pattern=north west lines, pattern color=blue] (4,4.5) rectangle (5,6);

\draw[line width=2] plot[ tension=.8] coordinates {  (2,2.5) (2,4) (3,4) (3,2.5) (2,2.5)};
\draw[line width=2] plot[tension=.8] coordinates {(4,4.5) (4,6) (5,6)  (5,4.5) (4,4.5)};


\node (v1) at (0,2) {};
\node (v2) at (0,5) {};
\node (v3) at (2,0) {};
\node (v4) at (5,0) {};
 \draw[->, draw=black, line width=2pt] (v1) edge  node[sloped, above] {time}(v2);
  \draw[->, draw=black, line width=2pt] (v3) edge  node[sloped, above] {spatial sites}(v4);

\draw[draw = white] (9,7.6)--(14,7.6)
node[pos=.5] {\large \textbf{Overlapping:}};


\draw[draw = white] (9,.9)--(14,.9)
node[pos=0] {1}
node[pos=.2] {2}
node[pos=.4] {3}
node[pos=.6]{4}
node[pos=.8]{5}
node[pos=1.0]{6};

\draw[draw = white] (9,7.1)--(14,7.1)
node[pos=0] {1}
node[pos=.2] {2}
node[pos=.4] {3}
node[pos=.6]{4}
node[pos=.8]{5}
node[pos=1.0]{6};    


\draw[ color=blue] (9,1.5) rectangle (14,6.5);

\draw[pattern=north west lines, pattern color=blue] (10,2.5) rectangle (11,4);
\draw[pattern=north west lines, pattern color=blue] (10,4.5) rectangle (11,6);

\draw[line width=2] plot[ tension=.8] coordinates {  (10,2.5) (10,4) (11,4) (11,2.5) (10,2.5)};
\draw[line width=2] plot[tension=.8] coordinates {(10,4.5) (10,6) (11,6) (11,4.5) (10,4.5) };


\node (v1) at (8,2) {};
\node (v2) at (8,5) {};
\node (v3) at (10,0) {};
\node (v4) at (13,0) {};
 \draw[->, draw=black, line width=2pt] (v1) edge  node[sloped, above] {time}(v2);
  \draw[->, draw=black, line width=2pt] (v3) edge  node[sloped, above] {spatial sites}(v4);






\end{tikzpicture}

==> other/phases.tex <==
\chapter{Physics of the $t$-$V$ model and Quantum Critical Behavior}
\label{chap:physics}
\textit{\small ``Nature isn't classical, dammit, and if you want to make a simulation of nature, you'd better make it quantum mechanical, and by golly it's a wonderful problem, because it doesn't look so easy.''\\
--Richard Feynman}

\section{The $t$-$V$ Model: Condensed Matter and Particle Physics Perspectives}

In this chapter we will give some more details regarding the physics background that motivates QMC studies of strongly-correlated quantum systems. In particular we will focus on the physics of the $t$-$V$ model, whose behavior is a key focus for many subsequent parts of this thesis. In addition to having interesting physics, it serves as an example of the success of Hamiltonian fermion bag techniques.

The $t$-$V$ model Hamiltonian consists of a free part and an interaction part. We begin by focusing on the free part, which is given by
\begin{equation}
H_0 = \sum_{\langle ij\rangle} -t_{ij} (c^\dagger_i c_j + c^\dagger_j c_i).
%+ 
%\sum_{\left\langle ij\right\rangle}V\Big(n_i - \frac{1}{2}\Big)\ \Big(n_j - \frac{1}{2}\Big).
\label{tbmodel}
\end{equation}
As before, $i,j$ are spatial lattice sites, $\left\langle ij\right\rangle$ denotes nearest neighbor site pairs, and the operators $c_i^\dagger$ and $c_i$ create and annihilate a fermion at site $i$, respectively. In the low energy limit, these quadratic terms can give the tight binding model of spin-polarized graphene in two different ways: (1) when $t_{ij} = t$ and the spatial lattice is honeycomb, or alternatively (2) when the lattice is square and $t_{ij} = \pm t$--the signs of $t_{ij}$ are such that every plaquette on the square lattice has exactly one negative sign--this will be referred to as the $\pi$-flux lattice. For both of these lattices, the free part gives two Dirac cones in the low energy spectra of the Brillouin zone \cite{RevModPhys.81.109}, as seen in Figure {\ref{cones}}.
\begin{figure}
    \centering
    \includegraphics[width=4in]{Pictures/brillouin.png}
    \caption[Dirac cones in the low energy spectra for the tight-binding Hamiltonian on a honeycomb lattice.]{Dirac cones in the low energy spectra for the tight-binding Hamiltonian on a honeycomb lattice. \cite{RevModPhys.81.109}}
    \label{cones}
\end{figure}

These Dirac cones in the low energy spectra make this model also interesting from a particle physics perspective. The linear dispersion relation and single layer of fermions in (\ref{tbmodel}) gives the physics of a single flavor of four-component Dirac fermions.

\section{Quantum Phase Transitions and Critical Exponents}


\section{Universality Classes and Renormalization Group}

